RL-Scope: Cross-Stack Profiling for Deep Reinforcement Learning Workloads

Deep reinforcement learning (RL) has made groundbreaking advancements in robotics, data center management and other applications. Unfortunately, system-level bottlenecks in RL workloads are poorly understood; we observe fundamental structural differences in RL workloads that make them inherently less GPU-bound than supervised learning (SL). To explain where training time is spent in RL workloads, we propose RL-Scope, a cross-stack profiler that scopes low-level CPU/GPU resource usage to high-level algorithmic operations, and provides accurate insights by correcting for profiling overhead. Using RL-Scope, we survey RL workloads across its major dimensions including ML backend, RL algorithm, and simulator. For ML backends, we explain a $2.3\times$ difference in runtime between equivalent PyTorch and TensorFlow algorithm implementations, and identify a bottleneck rooted in overly abstracted algorithm implementations. For RL algorithms and simulators, we show that on-policy algorithms are at least $3.5\times$ more simulation-bound than off-policy algorithms. Finally, we profile a scale-up workload and demonstrate that GPU utilization metrics reported by commonly used tools dramatically inflate GPU usage, whereas RL-Scope reports true GPU-bound time. RL-Scope is an open-source tool available at https://github.com/UofT-EcoSystem/rlscope .

==> Makefile <==
####################################################################################################
# Latex stuff.
####################################################################################################

DEPENDS :=
STYLE_DIR := styles/mlsys2021_style
MAIN_TEX_STEM := rlscope_mlsys2021
PDF := $(MAIN_TEX_STEM).pdf
MAIN_TEX := $(shell find -name $(MAIN_TEX_STEM).tex)
BIB := $(shell find -name $(MAIN_TEX_STEM).bib)
DEPENDS += $(BIB)
TEX := $(shell find -name '*.tex' | grep -v '/tex_arXiv')
DEPENDS += $(TEX)
FIGS := $(shell find -regextype posix-extended -regex '.*.(pdf|png|svg)' | grep -v $(PDF))
DEPENDS += $(FIGS)
PY := $(shell find -regextype posix-extended -regex '.*.(py)')
STY := $(shell find -regextype posix-extended -regex '.*.(sty)')
DEPENDS += $(STY)
# Make sure we are using virtual environment.
PYTHON := ./venv/bin/python
RUBBER := rubber

.PHONY: clean all arxiv arxiv_clean help

all: $(PDF)

help:
	@echo "$$ make arxiv"
	@echo "  Build uploadable *.tar.gz file for uploading RL-Scope paper to arXiv."
	@echo
	@echo "$$ make"
	@echo "  Build paper PDF."
	@echo
	@echo "$$ make clean"
	@echo "  Delete latex files and paper PDF"

#%.pdf: %.tex $(DEPENDS) Makefile $(BIB)
#	rubber -f --pdf -s --clean $<
#	rubber -f --pdf -s $<
#	rubber-info --check $<

$(PDF): $(MAIN_TEX) $(DEPENDS) Makefile
	$(RUBBER) -f --pdf -s --clean $<
	$(RUBBER) -f --pdf -s $<
	rubber-info --check $<
	@echo "Success!"

arxiv: rlscope_arxiv.tar.gz
rlscope_arxiv.tar.gz: rlscope_paper/scripts/package_arxiv.py $(DEPENDS) Makefile
	$(PYTHON) rlscope_paper/scripts/package_arxiv.py

clean:
	rm -rf *.aux *.bbl *.blg *.log *.pdf *.toc *.snm *.out *.nav tags *.tar.gz

# Remove same stuff as clean EXCEPT *.bbl to make arxiv happy
# (+ extra *.log.txt files)
arxiv_clean:
	rm -rf *.aux *.blg *.log *.pdf *.toc *.snm *.out *.nav tags *.tar.gz \
		*.log.txt


==> tex/custom_imports.tex <==


\RequirePackage{caption}
\RequirePackage{subcaption}
\RequirePackage{tcolorbox}
\RequirePackage{amssymb}
\RequirePackage{amsmath}
\RequirePackage{amsthm}


\RequirePackage[warn]{textcomp}

\RequirePackage{centernot}

\RequirePackage{graphbox}
\renewcommand{\baselinestretch}{0.98}

\RequirePackage{listings}
\RequirePackage{tikz}

\usetikzlibrary{arrows}
\usetikzlibrary{shapes}

\RequirePackage[normalem]{ulem}
\RequirePackage{enumitem}
\RequirePackage{siunitx}
\RequirePackage[nomessages]{fp}

\RequirePackage{xspace} 

\RequirePackage{comment} 
